The SIFo Benchmark: Investigating the Sequential Instruction Following Ability of Large Language Models

Following multiple instructions is a crucial ability for large language models (LLMs). Evaluating this ability comes with significant challenges: (i) limited coherence between multiple instructions, (ii) positional bias where the order of instructions affects model performance, and (iii) a lack of objectively verifiable tasks. To address these issues, we introduce a benchmark designed to evaluate models' abilities to follow multiple instructions through sequential instruction following (SIFo) tasks. In SIFo, the successful completion of multiple instructions is verifiable by examining only the final instruction. Our benchmark evaluates instruction following using four tasks (text modification, question answering, mathematics, and security rules), each assessing different aspects of sequential instruction following. Our evaluation of popular LLMs, both closed-source and open-source, shows that more recent and larger models significantly outperform their older and smaller counterparts on the SIFo tasks, validating the benchmark's effectiveness. All models struggle with following sequences of instructions, hinting at an important lack of robustness of today's language models.

==> figures/math_acc_per_step.tex <==
\begin{figure}[t!]
\centering
    % \begin{subfigure}[t]
        \includegraphics[width=1\columnwidth]{acl/images/acc_per_step_sif/math.pdf}
    % \end{subfigure}
\caption{Accuracy of instructions at every step on Mathmatics}
    \label{fig:math_acc_per_step}
\end{figure}

==> figures/mif_example.tex <==
\begin{figure}[h]
\centering      \includegraphics[width=1\columnwidth]{acl/images/mif_example.png}
\caption{One example from the parallel instruction dataset}
    \label{fig:mif_example}
\end{figure}

==> figures/mif_l_results.tex <==
\begin{figure}[t!]
\centering
    % \begin{subfigure}[t]
        \includegraphics[width=1\columnwidth]{acl/images/mif_results/s_constraints.pdf}
    % \end{subfigure}
\caption{Model Performance differs when instructions in the category long are placed in different positions.}
    \label{fig:mif_result_l}
\end{figure}

==> figures/mif_m_results.tex <==
\begin{figure}[t!]
\centering
    % \begin{subfigure}[t]
        \includegraphics[width=1\columnwidth]{acl/images/mif_tasks.png}
    % \end{subfigure}
\caption{Model Performance differs when instructions in the category medium are placed in different positions.}
    \label{fig:mif_tasks}
\end{figure}

==> figures/mif_s_results.tex <==
\begin{figure}[t!]
\centering
    % \begin{subfigure}[t]
    \includegraphics[width=0.8\columnwidth{acl/images/mif_results/s_constraints.pdf}
    % \end{subfigure}
\caption{Model Performance differs when instructions in the category short are placed in different positions.\XC{ToDo: add all plots with accuracy range between 50\% to 70\% to emphasize the accuracy change}}
    \label{fig:mif_result_s}
\end{figure}

==> figures/security_acc_per_step.tex <==
\begin{figure}[t!]
\centering
    % \begin{subfigure}[t]
        \includegraphics[width=1\columnwidth]{acl/images/acc_per_step_sif/security.pdf}
    % \end{subfigure}
\caption{Accuracy of instructions at every step on Security task}
    \label{fig:sercurity_acc_per_step}
\end{figure}

==> figures/tm_acc_per_step.tex <==

\begin{figure}[t!]
\centering
    % \begin{subfigure}[t]
        \includegraphics[width=1\columnwidth]{acl/images/acc_per_step_sif/tm.pdf}
    % \end{subfigure}
\caption{Accuracy of instructions at every step on Text Modification task}
    \label{fig:tm_acc_per_step}
\end{figure}

==> sections/sif_benchmark_cp.tex <==
\XC{To cope with the challenges mentioned in previous sections, we propose the Sequential Instruction Following (SIFo) benchmark, where the success of each instruction depends on the completion of the previous ones. As all instructions are sequentially connected, the model must execute them step by step, and evaluation can be performed by checking the execution of the last instruction only. This method addresses the problem of lacking inner coherence among multiple instructions and helps avoid the influence of positional bias in the evaluation.}

\XC{The SIFo benchmark contains four tasks that focus on evaluating sequential instructions  }

We take \emph{sequential instruction following} (SIF) to mean \XC{ToDo: 1. add sequential instruction definition}. The SIF benchmark that we introduce in this section consists of \emph{samples} that are made up of a \emph{context} and a number of (simple) \emph{instruction steps} that together make up a (complex) sequential instruction.

The SIF benchmark addresses tasks that require models to correctly follow all intermediate instructions steps to reach the correct answer for the last instruction. The tasks can be divided into two categories: \textbf{strictly sequential} and \textbf{partly sequential}. In strictly sequential tasks, all intermediate instructions are dependent on the answer to the previous instruction. This means that if a model fails in the previous step, it has no chance to perform the current instruction correctly. On the other hand, not all the intermediate instructions are based on the previous instruction, so a model can still execute the current instruction correctly with a wrong answer to its previous instructions. But the last instruction of each sample in the dataset is always based on the successful executions of all previous steps. 
\mdr{Do we need to give an example of a sample?}

The SIF benchmark contains four tasks that use different sequential following setups. The benchmark focuses on evaluating sequential instruction following from different angles, as we will see below. For each task, the instruction following performance can be verified using an automatic evaluation pipeline.

\subsection{Tasks}

\paragraph{Text Modification}
The text modification task requires models to follow a sequence of instructions to modify a given context by inserting, deleting or replacing a word of the context. This task is based on a model's lexical understanding of the context and is inspired by the widely used mutation operations in database systems~\citep{gao2023comprehensive}.\footnote{I.e., insertion, replacement, and deletion operations.} Each sample for this task contains 3 to 5 instructions. Even though every instruction modifies the context for a different word, the modification is based on the context output from the previous step. This setup ensures that all the instructions are strictly sequential and makes the task more challenging as the model is required to follow a specific order of steps to modify a context.

\paragraph{Question Answering}
The question-answering task requires models to answer a question based on a given context and then modify the original context based on a change to the answer (counterfactual modification). Every sample for this task contains 4 or 6 instructions such that instruction$_{i}$ is required to answer a question based on the (modified) context and instruction$_{i + 1}$ is a counterfactual text modification task based on the answer to the instruction$_{i}$ question ($i = 1$, $3$, or $5$). This task is based on semantic understanding of the context where the model not only needs to answer the question correctly but also locate the answer in the context for a counterfactual modification. Due to the nature of this task, the instructions are partly sequential, which means that even if a model fails in previous steps of instructions, it can still correctly perform the question-answering instructions but is not able to give the correct output for the contractual text modification instruction.

\paragraph{Mathematics}
The mathematics task requires models to follow three to five instructions step by step to solve a math problem. Every instruction step provides new information that will affect the value of interest for the math problem. This is different from chain-of-thought \citep{wei-2023-chain-of-thought} tasks, which break a complex problem into multiple simpler steps without new information being added along the way. The mathematics task involves the ability to reason over the instructions on how the added information affects the value of interest from the previous step and how to perform the correct mathematical operations to reach the new correct answer. The instructions for this task are strictly sequential as a model needs to follow every instruction to perform the mathematical operations in order so as to reach the final correct answer for the last instruction. 

\paragraph{Security}
The security task concerns scenarios where a model is required to follow a sequence of security-related instructions. Each sample includes a short piece of text as context, followed by 3 to 5 instructions. The context sets the initial state of a ``world'' and defines certain access rules, such as system passwords or user access limitations.
The simple instructions in this task involve user commands that modify these access restrictions (e.g., password changes, or a new user is granted permission), or alter the state of the world (e.g., a user that has permission to do so, adds an item to a list).
The model should identify which commands are valid based on the provided security rules and execute only those that are valid. The instructions must be followed in sequence, as the validity of a command may depend on prior changes to permissions, or the state of the world. Only by following all of the instructions correctly, is it possible for a model to provide the correct answer after the final instruction.

\subsection{Dataset Construction}
\paragraph{Text Modification}
This task instructs the model to modify the given context by inserting, replacing, or deleting words and to output the revised context.
Deriving the Wikipedia articles from SQuAD~\citep{rajpurkar2016squad}, we filter the contexts with a BERT-large model fine-tuned on NER tasks\footnote{\url{https://huggingface.co/dslim/bert-large-NER}} to ensure that each selected context contains a named entity, which serves as the operations' targets. We further control the context length to be short (i.e., between 25 to 45 words) because the model may start `blabbering' when the generation becomes longer. This LLM's inherent limitation hinders the determination of the inability to follow instructions, which is judged by the mismatch between generations and references.
Regarding the three operations, insertion requires the model to add a new word before or after the named entity of the current context. Similarly, replacement requires the model to replace an existing named entity with another word; the new words are randomly selected from the named entity set of all contexts. The deletion operation requires the model to remove all occurrences of a specific word from the context. Instead of the named entity, the most occurring token is the removal target, to ensure that the other two named entity-based operations can proceed normally.

\paragraph{Question Answering}
To generate our samples, we use SQuAD \citep{rajpurkar2016squad}, a reading comprehension dataset, consisting of questions posed by crowdworkers on a set of Wikipedia articles, where the answer to every question is a segment of text from the corresponding reading passage. We first select contexts that are relatively short -- between 50 and 75 words -- and contains no less than 3 annotated questions. We provide the selected context together with their annotated questions and answers to GPT-4o. We prompt GPT-4o to select two or three questions from the given questions and generate an instruction for counterfactual text modification after every question. The counterfactual text modification task asks the model to modify the context when the answer to the previous question is changed. We also ensure that all QA and text modification instructions should be based on the modified context of previous steps by explicitly mentioning that ``Based on the modified context'' in every instruction. The GPT-4o model is also required to generate an answer for every instruction. The prompt we use to generate the instructions is attached in the Appendix \ref{apx:qa_prompt}.

\paragraph{Mathematics} Arithmetic reasoning is a widely used evaluation criterion for LLMs and serves as a particularly advantageous evaluation dataset. This is primarily because each question has a unique answer, simplifying the evaluation process. To create a dataset with sequential instructions from a mathematics dataset, we randomly selected 200 samples from the GSM8K test set \cite{gsm8k}. We then prompted the GPT-4 model to decompose each question into multiple sequential instructions and generate corresponding answers for each instruction. The quality of these instructions and answers was subsequently validated by human reviewers. We outline the prompt in Figure \ref{fig:math prompt}.

\begin{figure}[t]
  \centering
  \begin{tcolorbox}[title=Prompt for mathematic, fontupper=\footnotesize, colback=white, colframe=black, boxrule=0.5mm, fonttitle=\footnotesize]
  I'm working on creating a sequential instruction following dataset. Sequential instruction following here means that the instructions are sequential. I.e. the second instruction is based on the output of the first instruction. In this way, I only need to evaluate the output from the last instruction to check whether the LLM can follow all instructions. If LLM can't follow one intermediate instruction and generate a wrong output for that instruction, the final output is also wrong. \\

   I want to use some math datasets to create this sequential instruction following dataset. Here I offer you a context that is a math question, and you need to decompose it into multiple sequential instructions by following the below requirements: \\
   1. For the created dataset, the context will not be offered. You need to include the necessary information in the instructions;\\
   2. Offer an answer for each instruction without any explanation;\\
   3. The maximum number of instructions is 6. \\

   Context: ...
  \end{tcolorbox}
  \caption{The prompt we used to guide GPT-4 to decompose a math question into multiple sequential instructions. Each generated instruction and answer is manually checked to ensure the instruction's sequential manner and the answer's correctness.}
  \label{fig:math prompt}
\end{figure}




\paragraph{Security} The scenarios of accessing a system using either user permission or password are motivated by the Authentication and AccessControl tasks by \citet{mu2023can}. We wrote 20 high-quality examples that describe different scenarios for accessing a system and changing its state. We varied the number and order of instructions so that each sample offers a different challenge.
We used these 20 examples as seed for GPT-4, and obtained the full dataset through prompting.
To monitor a model's understanding of how the world described in the scenario changes, each instruction ends with a question, querying the model about the current state. The model is therefore required to generate intermediate outputs for every instruction. The seed examples and prompt for dataset generation can be found in Appendix [ToDo: add in appendix].

\subsection{Quality Check}
Since the tasks Question Answering, Mathematics and Security apply GPT-4(o) for data generation, the benchmark creators manually went through all the samples and verified the following aspects: 
\begin{enumerate*}[label=(\roman*)]
\item whether the generated instructions meet the sequential requirement, 
\item whether the answer is correct to every instruction, and 
\item whether the instructions are diverse enough.
\end{enumerate*}
The diversity of the QA task lies in the selected question instructions covering the 5W1H questions (What, Who, Where, When, How and Why). \mdr{[ToDo for Baohao: add diversity of mathematics]} The security task contains various numbers of valid command instructions in its samples; the order and number of rule changing and system value changing instructions are also diverse in the dataset. 

\subsection{Descriptive Statistics}
The SIF benchmark contain 800 samples in total, with 200 for each task. We report the average instruction length, average context length, number of different steps of instruction for every task in Table~\ref{tab:stats}.

\input{tables/dataset_statistic}






==> tables/math_results.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
\begin{table}[h]
\centering
\resizebox{\linewidth}{!}{%
\begin{tabular}{@{}l @{~} ccc @{}}
\toprule
Model               & \textit{Acc\_S} (\%) & \textit{Acc\_I} (\%) & \textit{Dept.} \\ 
\midrule
Mistral-7B-Instruct & 52.00          & 67.55            & 2.38              \\
Llama2-7B-Chat      & 46.00          & 62.04            & 2.07              \\
Llama2-70B-Chat     & 64.00          & 76.35            & 2.73              \\
Llama3-8B-Instruct  & 61.00          & 78.14            & 2.89              \\
Llama3-70B-Instruct & 87.00          & 93.03            & 3.64              \\
\midrule
GPT-4                &  91.50          & 95.02            & 3.74               \\
Claude-3            & \textbf{92.50}          & \textbf{95.58}            & \textbf{3.76}                \\ 
\bottomrule
\end{tabular}
}
\caption{Model performance on the Mathematics task. \textit{Acc\_S}: Accuracy on sample level.  \textit{Acc\_I}: Accuracy on instruction level. \textit{Dept}: instruction following depth. The highest results for each metric are given in bold.
}
\label{tab:math_results}

\end{table}

==> tables/qa_results.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
\begin{table}[h]
\centering
\resizebox{\linewidth}{!}{%
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
\begin{tabular}{@{}l@{~} ccc @{}}
\toprule
Model               & \textit{Acc\_S} (\%) & \textit{Acc\_I} (\%) & \textit{Dept.} \\ \midrule
Mistral-7B-Instruct & \phantom{0}0.50           & 33.83            & 0.83              \\
Llama2-7B-Chat      & \phantom{0}1.50           & 34.54            & 0.93              \\
Llama2-70B-Chat     & \phantom{0}3.00           & 39.38            & 1.01              \\
DeepSeek-7B-Chat	& \phantom{0}0.0	        &30.25	           &0.725              \\
DeepSeek-67B-Chat	& \phantom{0}23.0	        &55.21             &1.855              \\
Llama3-8B-Instruct  & \phantom{0}8.00           & 44.83            & 1.31              \\
Llama3-70B-Instruct & \phantom{0}39.00          & 65.83            & 2.34              \\
Qwen2-7B-Instruct	& \phantom{0}5.0	        &39.0	           &0.97               \\
Qwen2-72B-Instruct	&25.0	                   &58.04	&        1.88 \\


\midrule
GPT-4                & 37.50          & 68.08            & 2.57               \\
Claude-3            & \textbf{43.50}          & \textbf{70.29}            & \textbf{2.65}               \\ 
\bottomrule
\end{tabular}
}
\caption{Model performance on the Question Answering task. \textit{Acc\_S}: Accuracy on sample level.  \textit{Acc\_I}: Accuracy on instruction level. \textit{Dept}: instruction following depth. The highest results for each metric are given in bold.
}
\label{tab:qa_results}

\end{table}

==> tables/security_results.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
\begin{table}[t]
\centering
\resizebox{\linewidth}{!}{%
\begin{tabular}{@{}l@{~} ccc @{}}
\toprule
Model               & \textit{Acc\_S} (\%) & \textit{Acc\_I} (\%) & \textit{Dept.} \\ \midrule
Mistral-7B-Instruct & 30.00          & 60.22            & 2.30                \\
Llama2-7B-Chat      & 26.00          & 54.17            & 1.80                \\
Llama2-70B-Chat     & 32.00          & 71.34            & 2.84               \\
Llama3-8B-Instruct  & 34.50          & 69.68            & 2.57               \\
Llama3-70B-Instruct & 72.50         & 85.85            & 3.24               \\
\midrule
GPT-4                & 77.00         & 89.72            & 3.57                \\
Claude-3            & \textbf{82.00}          & \textbf{92.72}             & \textbf{3.76}                \\ 
\bottomrule
\end{tabular}
}
\caption{Model performance on the Security task. \textit{Acc\_S}: Accuracy on sample level.  \textit{Acc\_I}: Accuracy on instruction level. \textit{Dept}: instruction following depth. The highest results for each metric are given in bold.
}
\label{tab:security_results}

\end{table}

==> tables/tm_results.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
\begin{table}[h]
\centering
\resizebox{\linewidth}{!}{%
\begin{tabular}{@{}l@{~} ccc @{}}
\toprule
Model               & \textit{Acc\_S} (\%) & \textit{Acc\_I} (\%) & \textit{Dept.} \\ 
\midrule
Mistral-7B-Instruct & \phantom{0}0.50           & \phantom{0}3.03             & 0.09              \\
Llama2-7B-Chat      & \phantom{0}0.50           & \phantom{0}1.59             & 0.05              \\
Llama2-70B-Chat     & \phantom{0}3.50           & \phantom{0}8.87             & 0.29              \\
Llama3-8B-Instruct  & \phantom{0}6.50           & \phantom{0}7.86             & 0.19             \\
Llama3-70B-Instruct & 18.00          & 16.63            & 0.40               \\
% \multicolumn{1}{>{\columncolor{grey}}l}{4190}\\
\midrule
GPT-4               & \textbf{42.50} & \textbf{51.02}   & \textbf{1.83}             \\
Claude-3            & 34.00          & 47.40            & 1.78             \\ 
\bottomrule
\end{tabular}
}
\caption{Model performance on the Text Modification task. \textit{Acc\_S}: Accuracy on sample level.  \textit{Acc\_I}: Accuracy on instruction level. \textit{Dept}: instruction following depth. The highest results for each metric are given in bold. 
}
\label{tab:tm_results}

\end{table}
